The Fission Barrier of Heaviest Nuclei From a Macroscopic-Microscopic Perspective

The concept of fission barrier - a parameter which enters in quantitative estimates of various observables related to nuclear fission - is presented from the point of view of theory based on the picture of nuclear deformation and energy dependent on it. We describe the macroscopic-microscopic method of calculating energy landscapes which is simpler than the selfconsistent mean field approach, and, due to its two-component nature, seems to be easier to adjust to experimental data. We present some models and methods used to find the fission saddles. For the purpose of illustration, we present results on fission barriers in actinides and superheavy nuclei, obtained within one macroscopic-microscopic model. We discuss comparisons with results of other models, including some of the mean-field type.

==> referencbak.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%
% sample references
% 
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{All references should be \textit{cited} in the text by \textbf{NameYear}. See the following examples:
\begin{itemize}
\item One author: (Author 1999).
\item Two authors: (Author 1 and Author 2 2007). 
\item More than two authors: (Author 1 et al 2001).
\item Multiple citations are separated by semicolons and listed first alphabetically, then chronologically: (Author 1990; Author 1 and Author 2 1995).
\item When two or more works by the same author have the same publication date, distinguish them in the order in which they appear in the text, with letters following the date: (Author 1997a, 1997b, 1996).
\end{itemize}
The recommended style for references (APS). Here are some examples. More on our \href{https://meteor.springer.com/project/dashboard.jsf?id=1105&tab=About&mode=ReadPage&entity=8644}{\color{blue}Project Website}
}
\begin{thebibliography}{99.}
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}, 33 (1995)
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, Clinical implications of dysregulated cytokine production. J. Mol.
Med. 78, 74?80 (2000). doi:10.1007/s001090000086
%Book chapter
\bibitem{phys-BookC} D.M. Abrams, in Conductive Polymers, ed. by R.S. Seymour, A. Smith (Springer, Berlin Heidelberg New York, 1973), p. 307
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
\end{thebibliography}
